Enumeration of nilpotent loops up to isotopy

We modify tools introduced by Daniel Daly and Petr Vojtechovsky in order to count, for any odd prime q, the number of nilpotent loops of order 2q up to isotopy, instead of isomorphy.

==> gap_code <==
#
# Counting nilpotent loops of order 2q, q odd prime, up to isomorphy or isotopy. 
# GAP script accompanying the paper
# "Lucien Clavier, Enumeration of nilpotent loops up to isotopy"
# January 26 2012.
#
# It was taken and adapted from the paper:
# "Dan Daly and Petr Vojtechovsky, Enumeration of nilpotent loops via cohomology"
# dated Aug 26, 2008. 
# The functions 'allSubsets' and 'NilpotIsom' were copied almost as it is in the
# above mentioned code. We thank the author Petr Vojtechovsky very much for his
# permission to use it.
####################################################################################


allSubsets := function( S )
# returns all subsets of the set S
    local x, all;
    if IsEmpty( S ) then return [[]]; fi;
    x := S[Size(S)];
    all := allSubsets( S{[1..Size(S)-1]} );
    return Union( all, Set( all, T -> Union( T, [ x ] ) ) );   
end;


NilpotIsom := function( q ) 
# returns the number of nilpotent loops of order 2q, q odd prime, up to isomorphism
    local m, divisors, dim, d, sum, size, idiv, subs, S;
    m := q-1;
    divisors := DivisorsInt( m );
    dim := 0*[1..m];
    for d in divisors do
        dim[ d ] := (q-2)*d;
    od;
    sum := 0;
    for d in divisors do
        size := 2^dim[d];
        idiv := Filtered( DivisorsInt( d ), k -> IsPrime( d/k ) ); # maximal proper divisors of d
        idiv := Set( idiv );
        subs := allSubsets( idiv );
        subs := Difference( subs, [ [] ] ); #remove empty set
        for S in subs do            
            size := size + (-1)^(Size(S))*2^dim[ Gcd( S ) ];
        od;
        sum := sum + size/d;
    od;        
    return sum;
end;



NilpotIsot := function(q)
# returns the number of nilpotent loops of order 2q, q odd prime, up to isotopism.
# see Thm 6.10 in the article for a justification of this computation.
	local sum;
	sum := -(q+1)*2^((q-2)*(q-1))+(q-2)*2^(q-1)+3;
	sum := sum/(q^2);
	sum := sum+NilpotIsom(q)+1;
	return sum;
end;



Count := function(qmax)
# this naive function prints the result of NilpotIsot for primes q less than qmax
# so as to be usable directly in a LaTeX written article, or to fit on a simple file.
	local q;
	for q in [3..qmax] do
#		if IsPrime(q) then Print("$", q, "$ & $\\np{", NilpotIsot(q), "}$ \\\\ \n"); 
#		fi;
		if IsPrime(q) then Print(q, " | ", NilpotIsot(q), " \n"); 
		fi;
	od;
end;



==> order_2q_isotopy_upto100 <==
odd prime q<100 | number of nilpotent loops of order 2q (can take several lines)
--------------------------------------------------------------------------------
3 | 3 
5 | 64 
7 | 3658004 
11 | 1023090941561683953759580 
13 | 2684673506279593406254437209960379084 
17 | 382103603974564085117495134243710834769544696954218618882023686506660 
19 | 
200631428878742858604463718156663900134339768107896670630238205955592093079613\
51527455884 
23 | 
102324502997587414459186469053420401193074927423105508675476331185576728031952\
5492343881308456768734437163298876113088718585209350360276 
29 | 
160961753600349400106317445398936496901865630954913796746589997652116462489679\
582985550624906756951346560554453774007519598258710976122226347100655327618826\
61565638302718622075219306227029003466240587334063716826344947522796 
31 | 
273055912808904521274444559546524957426529296828503788431341138798762301540236\
680797525619021386387721285236878967107706256403369177026689699898862067160533\
606032838906000521204005731761902653260783673795407303561154781048628841656356\
156600908620283824710852 
37 | 
402799189227707657580086586290345314584695299118786943541056588737083135808479\
215967481585516182468763639749231543656198610707436521391945921667717044275531\
768958644984177741425935187387570207583989916334557869203617737881513754555339\
084876316427247894644695695381920287806299638771415672623088712986498563818030\
566233836695726262310808140602705410578671369897352409735354556 
41 | 
601402918113301289138128340340926948069223340763331050056138635041734999320824\
897785790957344053418529898977644675412375594912967509078458194726212585498374\
996859436658043319854669265469270861678797856571286037074292729216013842454841\
329658229846887381753901506994354542541333503797270545023337326035383601362211\
994944921102906471176932187764861937387516853958206480928905988038814247716024\
976233530141249443030581580377001560646505435632528208830963442473443356500 
43 | 
304415198648442848372280370932270077420644016267955973354695776551503538824098\
172941579980565833629724928453969072020035885358147626611947826438506231240478\
823715623974960581796296197320403294829255940867990442655588785757161697287489\
260592402768661693866377660869430709982626059593704347515413624570094577385972\
666705652603781171614106985420361769042026397277790557908968685339472929490183\
132227059702543945359539508374312305068791684251623706795247504513031753642887\
3918268125106869473098704730605610907093706012 
47 | 
133394362817056747264567490852436804168223415675003772647371854614569223874243\
854434330500392816149381387844685148267513094911767495759120114169915471381482\
557516259044206543499529810287214674543018808172992745229883306148583477290283\
447326585163418140652350585332023526879692869284014491414462040521087361699097\
229043684168091519195080674400579566948385530700516041099676299466763410138428\
489066088494140125762977770668354539332218006009892756396671332750709145362786\
486317153161080182440820702599570359974176426580730602243355280159419602478123\
2357688136493184596104961392954527357401777486793672437134486098368762404 
53 | 
146890401547253714985465147356625579949165317489771313008236718517802224786946\
148345279603403874096968762932391541262545861587509445404921353495104174019774\
701668280644687217993333754344910608340858587040771502724271024776321182497328\
069204028781924748317228008758263311254273007538864363860882822335140109840612\
101571884998681225143674027179504718282112673182734970394255185323191347331136\
035898243354668137286284025645548036675388598348130660930292505544128612728340\
700848277437441608589763064966657345086365780128468327544715509253952061752535\
675795952760992607567358578945609912883044755674525309005047889618982930209733\
748452755341599436662900798910427448396233947772511488800278729182283683411413\
707452831286578739445634957596173907332364063165112076269626356330794577257582\
57296783033820 
59 | 
794389780083748528419640584786869106094994690582328185346797396839381594132641\
460918432440357826690492968810229860734718354871262791964805123256109839756420\
042046258182762395477371079542181346402883643204440738970019883692948773963370\
634074779269438609265111032846170827782703088714463662100141320879930064040953\
922997551440338498998921957278581158091653346464492526938606089626865789143262\
938253835842831306811989774821286560104676533347949984041987975937419344348596\
206336711846107093939352117828693620770851909144937841484529519591906630464850\
648362637543215717212666386952080769633239631341177360571143760053230580811652\
082712976902082656104694853049169374362988387023148302096294514528382304337493\
412544326731887758249104610690927937270010864871235777281700169626914430734358\
492407452980440800994136259039295642978956615257831448563062713797584717316350\
676385381035340508637378560800480237503266742484301033327024680172863619567245\
375622095870555345834304472543103987381682842592666620 
61 | 
198323295354225275925242438658298226192977674310847064434603841437562973969663\
940319565152208917895991068757823700525429367083416814869816670119406895448776\
474245257717284211538687147799064825621569597948889835830841059873373569824860\
772738473916107865320043753523968927486189345058486060042044571122448382497520\
289095449545480409375270945116301420515676252318400785553745810099140816304142\
391162136639145482250880577684084274291370316589575651510996977880274017524757\
592478709573812571669496057706165360504487353467820164339419304772950157208670\
840022880327258094276577216698377938622444008581788351053669628134366436828305\
642205839544736782862789382162218154171916529951288700738054944905724190551631\
713247074931978770532416886097594221026998945291563809266839431114914488757229\
674706478985188199020335308100507046381331100345419628180730335905716291774754\
468715893538957072844842327457197484613579240244667810462891631308404737105205\
981505480333035161908267201462088385455379066471544910036080312745854711663987\
75079936290496724246251681312578464056095364908 
67 | 
885090863178956498643936836975772994379843101777232437397117391003491106846696\
505484057985224849619873480278849963574328236936220030481994568703150803631916\
669636238891142039756472559144236389323754816231523423576383280997350801166301\
905020303034137180958669910223825858069917191032803642092498047451640420731629\
655587146135571432270418467774368653239896758159698827089092470167476208330628\
701216675738424205771966589648074114092202406932992523182961423418033497454824\
998916960591084893685121813169286252741778375022289696621498507420010300687006\
099019905969837017411835849837789429042455872135128890721681886089757379831116\
339275507675402025432793724932974423194094084047620361499350183593519666237749\
286765068765768813495026585448315699455098936052934335042448562606622314637926\
030090372506173643349421939073303824900394612389120426178166642097420364891612\
576018675997409318984891380896135395015302899552746962313017521124784388717844\
836236672023212658545468177845082690298195992211499047777859163033289652471978\
903843863421850342865403286222597289815905160189056220398537994154168140431831\
630828629070015283393768722956374033713609343196844843930793990994280971696826\
299506585427233594986554484523553413440935935581143648286186265757416052606658\
24638189063543883134424907128461794860 
71 | 
267463374448870477908904749316438425681161382173738829845947189179720304191825\
634021638268248050680254362930238635507976480869757490183299379414775862452491\
056299978637767721011243523924278492008388730454825921962838694127868410608784\
255438472506106184140761808341939680169652931876348788542870211356385691340164\
869824590316866184308540122043495619624885064200835656631397562253839611603485\
850689372686818614335486728961391356155160425728452614049662933996259954796217\
306176947578112295192916187567491620635196430127857559075431306097241668665564\
164919016813422457931774722887607886224813276651714383398389340753837045523989\
094821939820454776220185208099078789083560345490597640576456853498502395167212\
231429672192884213583871646609288205850180874260655781654175596630884300253464\
514872673106813136086776631215790144222804679526762584091507297515946063047893\
632866613073001548671195193438164007855332266798611435832872689528407530410530\
770779400845950701991203857164720945130386077367356670983560420088369428995281\
893826523954321359341143237278227930522862744160088507783963832023995732674759\
779682975782955957145778168380207597873528459753103027907641558367093070662749\
794461389781589336530647670744322643127434673211566494606437838902378026546257\
169489271698631353119083267608436166789452506190489723799323343287687292492460\
667029566295881181372772767691117846266860313518649110789763428243629915942566\
521910474480299391300431717223347829636923380 
73 | 
191143536773669054600599679585380640561624542810935748338801778875821343375150\
171428491420259768679616349953508242853612305930996035112853077155277625077810\
539779421707856210150093602696033653401743267578329807358996642244118353179009\
296333582613469142917249853730674022341715681349056653600840500547944656686787\
640823611046208760200921680007209104196407316936794047147794251468997387868098\
663906743920572187868368672520331387951265520244881594217959424744985981329868\
560817189161539756852169144881061848942059186716993017181144113416061463301418\
191620706224005650994797626068362761943029025357023897237701775730402964472859\
367839722260009872274908477741421083112246012279537954800313115914833862390680\
905292083359082875455190085500659533139909904756127802957340705827298405910420\
201653309291632761438842414034024246745584642371861515479247485505762172352103\
518265611962920242416340781048610761966255471545875057202669099033661188856918\
566075049330075800440240075201763671666359503964587262483074181222616711234663\
084687005405526481742775519417126989374274120404784493454670448455509888098817\
367976961471056348341178429619236374880290094273428608295393325954553020451560\
198097611726128174670915311449689862369553311625514926085054947422549247980914\
631026828261543667210686376504745711683419019635020780609007485192197199341799\
340049422180466919014347476330331197790515363769261442075615849694827114754611\
440879540527072966847868764641273394689236875215540137474447011788135645393032\
9459399368913831045777835197501402486505260739611796 
79 | 
198978050993371321658795320254152821390192381283022856637720209749014818564554\
764433488166203023342685767778654825385744463800419362733209390695666307371502\
447510468322771348498344620297026040626368925729117470088499864297917792484254\
913271810864575894843631718836079404409263757786305890124410200975714483021926\
609431167238485642755272359572000549263761364263741788468264846326830906118651\
379476764604809673393409001972069393241685448976276188044420092319202220136203\
341591670892618978874928182475170209003070389907797940237461419400174572238153\
503231646022946395863235505540808519059430087293250043558318610889248186406443\
818183945705423565707296919813026259778955552087396637409259811159754974184629\
801026143164911750283952667959484444960254613724072432527943985277940380563695\
649460646272284861718796237426991400569032413266850247822806212305429767891552\
501958980250911633471587572454379104077271090660930957787303652859826154524142\
705470864849346887942615381349063510693526208850897129693184045157519697494406\
844211733707763920016829056990040321473149583861453773032817698340009078779884\
098385013862650463382182787920593436446978791887016281574498513685621910717077\
035409429354781477194214730655442627530451291428141280084878415505424991178134\
826303400055606729682557913031822188652760137012339001959136216971780747077957\
027651516953144952046607644893241584851337810683231136764613204238656285543616\
030815655413186976524769864637791260834086526896039794680973767727688966874490\
167383293147720187257539896968212213300366487122152086750480973325592223555850\
300820325302278502983737068981408940245315565294001868213488780769744664957131\
374045392522909702287493884889268869713003329399480924793678609268441403149754\
008758100732993503745642911770077068251620972006716765982134570972699930378072\
095564516 
83 | 
488946298856159294647608768977949871407244478200090771990648483083536556338078\
498371718513135267918393895612778246462866286019675700868701676877016227234255\
519062759386307942732743906793918995799407392215998903503365206816068787802222\
291839216203752858903432568728038779153366734807898610957678510498151800756142\
704062643421503821649017548043202563950232493390021849664175569544708230899855\
940490432208122930841060961442502617704144393759362447562789660886430492453727\
477437259450899786352650040433082644998521383270435472883442070523645260452949\
197909484335335305087746245275308586617278662022307454369522536350515857720668\
932091470895062962972788513081765407009739835303666725443256112088331564768487\
774360616701422915727386536530432567609201121062964117898035263887525093623317\
118699596191213378149086773540927483591875472131174889709373708635220864296890\
315976382978475029202646438540276257072059413772345108683952680399773762149434\
996675383089448625290537427599114550560844445958074105861286740232452917815836\
599855470454958610126280009005561809253380940221487263124457750538756782120234\
010438525697911558969595542643134963143218645053682021463479788536610107225757\
713333647846962470642731374919294756950591990126379698555857672549485811366769\
541831275053809358336656653341804311358980599905644192627374860825484514707305\
685865919369085002961282407311977494989939722468806927902503051569177740562122\
264368237774391602045774999196920912438501969041524111688343550382923159078368\
325100915293315458705923276706502265884595927753261003820986974962808982339793\
399877545680485106195338738162950874726584876177015968807367092386726367440640\
088290579653948136782941580019663420499016167367162438201604974552909029061480\
075889352563650410944771680185907440436124658197974182998141279872666493966636\
844962308545342906995736492578525823142376211374573616171810887123850796106124\
999018836940773974912930897784429830548339812829333496454539236935511477593355\
83590383717936738941195949082949452280436748 
89 | 
695639313772535794430200748830640795060353869748921391502600099545866362575521\
114455977493970593490897801672690989978455252563819539460965315560572422832199\
692841286109063660376761442887527760839265744200172166468570878585321901479109\
063126018457167043844551588317829050050374002306531215961357699882220884177702\
918221253534044405274646362017771254613433525401457557857622085911798346004450\
283365485978015232766349960774221116357515277857718970488875943157787486137741\
549225927878385097948036484060046563882410593242020314775539467403966233339270\
709111863201085583718534768685172810777725075721662897140001163972179374574523\
659605921543652544348261511255932661850981543119343797626648260841986273338544\
198612329492762627849070054265112408669089052011285181404455130545167030330001\
983172351944737187151167853268272506020587065657283761219055677547904108504301\
497450974902891517596277335870855851474362283685979986343713520961557261025157\
226451156056797457509162508076948718482095531019259875990153843500309122877233\
244338159489069882410813821357427697796619932683898691684892332642004188806820\
592775967995929061036243596457382892482797535225186394783823852934175862521239\
219827039170600033604097861944612743076256407363572588611557560951401892170369\
792318201029110381034726333654969549481769094230758899891476341799842845458626\
833368662064487881878076927086959585684525620341429227299640119190572907084090\
818671304694971660195711011557242715479722299183725142288064220297088131045508\
045818785991902565336606858667666996738800800912166236219992678177894437281307\
021196614982039923915897862252268073831882648465309875385296925260350449610244\
544974331936720951571434415054824180674750211280397663229440170737555927532372\
092096929036169387685771033188962044346365231859362778381322438725703519541627\
453243160122794437367452239401804065442073329791266043006855046368766438652944\
160585981839823483410848281967864526976784920655995355077652622143155080525041\
001810877168485482871531128564958386491686784077007982890721632329546542538655\
164867763641857172034810375737416203140970017300185709306881875777618109749692\
150691882238244141668071417610197175973312760020917896549584353055614634073817\
485742837597335456822625496320649748893218806115077102196794577283864498521258\
4750770092058181818130149805694072372 
97 | 
273996966051927736939875082698520805718160881725669429809682322173525292572558\
804194386123563036406562255254693905936415114853468262550739525674135289434013\
798938716213291360787120155654780088474799507944795068223106836256401072307626\
817542706937334805679720951858563366947794155016536963089311835980734672439320\
846265332179651046951471769323292041406160262120072805737363353878446873162480\
674846145875023050720377170952751592437284839109214313979297743009480986371179\
777141242229778967123804839486294728931155941412744998772124140083398888241574\
373725361345656915017403826033708123241378022462765597993512185855157671289653\
448108327953511654354441297537278770089352585719200707198433744792189490370978\
128620472410871070417908557206984483521104212162604939677215991612867007277542\
319112830908965324541485277242145047915599742062802707144035351378633221552374\
345155885025055443033950622448580257549661947190171334974125386206665153971184\
094907631963107009798127572904387246048592842442339884663686121749275953309504\
199420099857428429426920211121782557813310787382997392130406832765197047018495\
225145308012215132782213276008840147610393098267699781932815195884286543599047\
896040303285093587565971127500793844887286635378987053018210177798632035568799\
364688196714297202696296665677162738471068780623233836746974576414184117996930\
536369655240212247021108332618231507447146009319582567349533167331483128113685\
339142692969136734841996317572760596333526654523241402442606724978601266079967\
973556386957205401837307132610416074131362951191205517840553827068720487585251\
897129722079831065595975073123504066581837782485361419886407679319148394525075\
379500540022999537254865921888390379808778277496768102330827862110172949926685\
040718885213518504126070218077461884881598723588630442146767714401870585931687\
276004265888726683395919760116147172770317675832547433978212725223446612241822\
254688284053038043137131329968498678013955557902901507369272734972693293350946\
729605819588862902735374683842442410225569310182232037625490952252856888464324\
078795875545421135965282751645731202208304464931967690233315609693791473096641\
846620122813762099809970698530569772006781418923577374251649285545480281990139\
319981872351082448437184265082302897548579238702452290353664161698648532320497\
926017671959012981882821200789345959469155531847718841979899155342630428196809\
454821915494113484967364963069292144131731480115318498128907068100883807826135\
065109607032685005079042884770744988889590090876531652329050028406536113808753\
477639562331747183917324320972295631716536808228557597395201939431359186170988\
351950155123186335822971267183053523451139316873549621916624048594719583184675\
010723717049084529309388253471255537985699571889046331590416560583272855765835\
9599153604 


